Estimation of Passenger Route Choice Pattern Using Smart Card Data for Complex Metro Systems

Nowadays, metro systems play an important role in meeting the urban transportation demand in large cities. The understanding of passenger route choice is critical for public transit management. The wide deployment of Automated Fare Collection(AFC) systems opens up a new opportunity. However, only each trip's tap-in and tap-out timestamp and stations can be directly obtained from AFC system records; the train and route chosen by a passenger are unknown, which are necessary to solve our problem. While existing methods work well in some specific situations, they don't work for complicated situations. In this paper, we propose a solution that needs no additional equipment or human involvement than the AFC systems. We develop a probabilistic model that can estimate from empirical analysis how the passenger flows are dispatched to different routes and trains. We validate our approach using a large scale data set collected from the Shenzhen metro system. The measured results provide us with useful inputs when building the passenger path choice model.

==> Background.tex <==
\section{Overview}
\label{sec:Overview}
\subsection{Metro System}
In general, a metro system is composed of some lines that are composed of some stations, as shown in Figure~\ref{fig:side:metro} which is the graph of ShenZhen metro system. Be noted, in this paper, we refer to the metro line with direction and indirection as logical metro line and physical metro line respectively, e.g. the metro line 1 in Figure~\ref{fig:side:metro} is physical metro line, from JiChangDong to LuoHu or from LuoHu to JiChangDong of line 1 are logical metro lines. If not particularly pointed out, a metro line means a logical line in this paper. There are two kinds of stations: general station and transfer station. A general station is for one physical metro line in a public transport system, while a transfer station is for multiple physical metro lines that allows passengers to change from one line to another. A platform is a place where passengers waiting for a train and identified uniquely by a physical metro line and a metro station. In general, a passenger waiting on a platform would get on the first arrival train with enough capacity at his/her waiting platform, if the train don't have enough capacity to accommodate all passengers waiting to board, some passengers must wait for the next or other later trains.
\begin{figure*}
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.2in]{./allfig/metro.pdf}
\caption{Metro graph of Shenzhen}
\label{fig:side:metro}
\end{minipage}%
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.2in]{./allfig/trip.pdf}
\caption{Segmentation of a one-transfer trip}
\label{fig:side:trip}
\end{minipage}
\end{figure*}


\subsection{Segmentation of a trip}
A general trip of a passenger in metro system can be depicted as 5 steps as shown in Figure~\ref{fig:side:trip}: (1) passes through entry gate and walks to the platform, (2) waits on the platform for a train, (3) boards a train and stays on the train until the train reaches the passenger's destination,(4) gets off the train and exits the metro system. To be noted, if the passenger needs to transfer, before step(4), transfer between platforms needs to be considered. So the whole trip duration is composed of: entry time ({\it ETT}), wait time ({\it WTT}), on train ({\it OTT}), transfer time ({\it TFT}), and exit time ({\it EXT}).

In this paper, we denote the minimal walking time of $ETT$, $TFT$, $EXT$ as $ETT_{min}(l, s)$, $TFT_{min}(l, l', s)$ and $EXT_{min}(l, s)$ respectively, where {\it l} and  {\it l'} are metro lines, {\it s} is a metro station. The method for calculating the value of $TFT_{min}(l, l', s)$ and $EXT_{min}(l, s)$ has been given in our previous paper~\cite{Zhang2015Segmentation}, which first use non-transfer trips with only one route to derive the minimal walking time between the gantry and the platform, then use with-transfer trips with only one route to derive the minimal walking time between two platforms.


\subsection{Assumptions}
We use two assumptions in this paper:
\begin{itemize}

\item For simplicity, we assume that the enter time or exit time must be less than the departure interval between two adjacent trains. This assumption is rational, because for most metro system, the distance between gateway to platform is not far.

\item We assume that a passenger inside metro system would not intentionally linger, that means a tap-in passenger will board the first arrival train with enough capacity and exit metro system after getting off the train that reaches her/his destination as soon as possible.

\end{itemize}

\subsection{Data type used}
In this paper, we use two types of records:
\begin{enumerate}
\item \emph{Smart card records}: A smart card transaction record $sr$ is reported when a passenger passes through entry or exit gate by tapping smart card, which includes fields $sr.id$(unique identifier of smart card), $sr.s$(metro station), $sr.t$(transaction time) and $sr.tag$(21 tap-in, 22 tap-out).
\item \emph{Train operation records}: A train operation record $tr$ is collected when a train arrives at or departs a station, which includes fields $tr.sq$(train sequence), $tr.l$(metro line), $tr.s$(metro station), $tr.t$(transaction time) and $tr.tag$(1-arrive, 2-leave).
\end{enumerate}

\subsection{Modeling}
Travel time of passengers depends on the interaction between passengers¡¯ route choice behavior and train operations data. For each passenger of an OD pair, we can find all plans chosen for every effective route by matching smart card transaction data with train operation data. If we know the possibility of these plans, the overall probability of each route being chosen can be calculated easily, to get the possibility of these plans, we transforms it to calculating two kinds of time-dependent polynomial distribution about passengers' train chosen behavior, one is the number of trains needed to wait at their original stations, the other is the number of trains needed to wait at transfer stations, To do it, our intuition is that there are a significant portion of passengers with only one effective route and need less than one transfer, their trips can be used to calculate two kinds of time-dependent polynomial distribution. Accordingly, we firstly find all effective routes for an OD(origin-destination), then for each passenger, we find all possible plans he/she could choose for each route, in the next section we give an probability model to calculating the probability of each route being chosen for an OD with multiple routes.


%In this paper, we define a trip as a travel of a metro passenger, which contain two smart card records, tap-in record and tap-out record.

%For a trip, we divide a passenger's whole journey into several parts by the metro lines being chosen, eg,


==> Formulation.tex <==
\section{Overview}
In this section, we give an overview of the ways to analyze passengers' route choice behavior. We first present the assumptions and notations we will use in this paper, and then give a probability model which can be used to calculating the probability of each route being chosen for an OD with multiple routes.

\subsection{Definition and Assumptions} 
We use three assumptions in this paper:
 \begin{itemize}

\item For simplicity, we assume that the time a passenger walks between the platform and the entrance/exit where he taps his ticket is less than the departure interval between two adjacent trains. This assumption is rational, because for most metro system, the distance between gate to platform is not far.

\item We assume that most passengers will passes through exit gate as soon as possible after getting off the train that reaches her/his destination

 \item We assume that for a given threshold $\delta$, the probability of each route being chosen for an OD with multiple effective routes is stable during time interval $[t, t + \delta]$. For instance, if setting $\delta$ as a half hour, one day can be split as $I=\{I_1,I_2,I_3,...,I_{48}\}$.
\end{itemize}
 
 
 \emph{DEFINITION 1}: A passenger $x$ in this is associated with a begin time $x.b$, origin $x.o$, end time $x.e$, destination $x.d$.

 \emph{DEFINITION 2}: $Tapin(s,l,j)$ represent the passengers who enter metro system at time slot $j$ in station s and chooses metro line $l$.

 \emph{DEFINITION 3}: $Transfer(s,l,j)$ represents the passengers who transfer from metro line $l$ to $l'$ in transit station $s$ at the time slot $j$.



To estimate the density of passenger flow of trains in every route, we need to identify the travel plan of each passenger's trip. Here the travel plan of a trip refers to the chosen route and trains that the passenger gets on.
For all the passengers of an OD pair, we investigate the portions of different plans that the passengers choose. The portions are then considered as the empirical distribution of the probability that a passenger chooses a plan for his trip on the OD pair. By computing the distribution of plan choice for all the OD pairs, with the knowledge of the number of passengers on each OD, we are able to estimate the passenger density in every train on every route. In the following of this section, we give an approach to get all routes for an OD pair firstly. Then for each passenger, we find all possible plans he/she may choose for each route. The solution to calculating the possibility of each route being chosen for an OD with multiple routes is given in detail in the next section.



%
%For all passengers, we can analyze their route choice behavior combing smart card transaction and train operation data. There are two challenges for that, firstly, given a trip of a passenger, how to find all possible trains or train combinations that the passenger may board for each effective route, where trains and train combinations are for the passengers who do not need transfer and need transfer respectively, in the following section, we refer to them collectively as plans. Second, if there are more than one effective route that we can find corresponding plans the passenger could choose by matching the two types of data, what is the probability of each route being chosen.
% Accordingly, in the following, we firstly find all effective routes for an OD(origin-destination), then for each passenger, we find all possible plans he/she could choose for each route, finally we give an probability model to calculating the probability of each route being chosen for an Origin-Destination with multiple routes.
%
% For each passenger of an OD pair, we can find all plans (trains or train combinations) chosen for every effective route. If we know the possibility of these plans, the overall probability of each route being chosen can be calculated easily. to get the possibility of these plans, we transforms it to calculating two kinds of time-dependent polynomial distribution about passengers' train chosen behavior, one is the number of trains needed to wait at their original stations, the other is the number of trains needed to wait at transfer stations, To do it, our intuition is that there are a significant portion of passengers with only one effective route and need less than one transfer, their trips can be used to calculate two kinds of time-dependent polynomial distribution.

\subsection{Finding all effective routes for an OD}
\label{subsec:effectiveroutes}
In this subsection, we use two steps to find all effective routes for an OD(origin-destination). The first step is to find all routes for an OD pair; the second step is to filter the routes that may have never been used by passengers from these possible routes. We use the algorithm proposed in~\cite{Eppstein} to find the $k$ shortest routes with efficiency in time $O(m+nlogn+k)$, where $n$, $m$ are vertices and edges in a digraph respectively. We simple define the cost of a route as the  minimum time cost that contains the minimum of walking time and the minimum of of running time of trains. The $k$ can be determined in terms of the accessibility and complexity of metro system. In practice, not all of the $k$ routes of an OD are used by passengers. In order to filter those routes that passengers never choose, we sort all trips of an OD pair over two months by the time cost (the time difference between the tap-in time and the tap-out time), and filter the top $Y\%$ trips with largest time cost.

Although most of passengers do not linger too long inside metro system, there are still some passengers showing abnormal travelling behaviors, such as beggars, express logistics worker. Their time cost and travel plan choice may be anomaly. Our recent work~\cite{zhao2014understanding} found that the optimal value of $Y$ is 2, which can filter the abnormal passengers with high accuracy. Then we get the largest time cost denoted as $C_{max}$ of the remaining $1-Y\%$ trips. Finally we filter the routes with time cost longer than $C_{max}$ from all possible routes. The rest are effective routes. In this paper, if not explicitly pointed out, a route refers to an effective one.
%A recent study~\cite{HAnalysis} concluded that 40 percent of the commuters used only one route for their commute and the remaining 60 percent of commuters used two routes at most, accordingly,    In this paper the $k$ is set to 3.
%in this paper the $k$ is set to 3. In reality, not all of the $k$ routes of an OD are used by passengers, in order to filter those routes that passengers have never chosen, we sort all trips of an OD over two months by time cost(subtracting the tap-in time from the tap-out time), and filter the top $Y\%$ trips with longest time cost.
%That because although most of passengers do not linger too long inside metro system~\cite{zhao2014understanding}, there are still some passengers abusing metro, such as beggars, express logistics worker, their time cost may be anomaly. Our recent work~\cite{zhao2014understanding} found that the optimal value of $Y$ is 2, which can filter the abnormal passengers with much great accuracy. Then we get the longest time cost denoted as $C_{max}$ of the remaining $1-Y\%$ trips, finally we filter the routes with time cost longer than $C_{max}$ from all possible routes, the rest are effective routes. In this paper, if not explicitly pointed out, a route refers to a effective one.

\subsection{Extracting all possible plans chosen by each passenger}
\label{subsec:possibletrains}
In this subsection, given a passenger's smart card data and train operation data, we find all possible plans chosen by the passenger. A general trip of a passenger in metro system can be depicted as 5 steps as shown in Figure~\ref{fig:side:trip}: (1) passing through entrance gate and walking to the platform, (2) waiting on the platform for a train, (3) boarding a train and staying on the train until the train reaches the passenger's destination,(4) getting off the train and exiting the metro system. To be noted, if the passenger needs to transfer, before step(4), (5) transfer between platforms needs to be considered. So the whole trip duration is composed of: entry time ({\it ETT}), wait time ({\it WTT}), on train ({\it OTT}), transfer time ({\it TFT}), and exit time ({\it EXT}).

\begin{figure*}
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.2in]{./allfig/metro.pdf}
\caption{Metro graph of Shenzhen}
\label{fig:side:metro}
\end{minipage}%
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.2in]{./allfig/trip.pdf}
\caption{Segmentation of a one-transfer trip}
\label{fig:side:trip}
\end{minipage}
\end{figure*}

In this paper, we denote the minimal walking time of $ETT$, $TFT$, $EXT$ as $ETT_{min}(l, s)$, $TFT_{min}(l, l', s)$ and $EXT_{min}(l, s)$ respectively, where {\it l} and  {\it l'} are metro lines. {\it s} is a metro station. The method for calculating the value of $TFT_{min}(l, l', s)$ and $EXT_{min}(l, s)$ has been given in our previous paper~\cite{Zhang2015Segmentation}, which first uses non-transfer trips with only one route to derive the minimal walking time between the gantry and the platform, then uses one-transfer trips with only one route to derive the minimal walking time between two platforms.

Let us denote the arrival and departure time of a train $tr$ at station $s$ of metro line $l$ as $T_{arrv}(l,s,tr)$ and $T_{lv}(l,s,tr)$ respectively. Suppose a passenger $x$ enter metro system at station $s$, he being able to board the train $tr$ needs to satisfy the following Equation~(\ref{equ:condition})(i). Likewise, if a passenger $x$ exit metro system at station $s$, he/she being able to board the train $tr$ before he/she exiting metro system needs to satisfy the following Equation~(\ref{equ:condition})(ii). For a transfer passenger, let us denote the arrival time of a train $tr$ at the transfer station $s$ of line $l$ as $T_{arrv}(l,s,tr)$ and the departure time of another train $tr'$ of another line $l'$ at station $s$ as $T_{lv}(l',s,tr')$. That the passenger getting off from $tr$ could board train $tr'$ needs to satisfy Equation~(\ref{equ:condition})(iii).

\begin{equation}
\begin{split}
 &(i) x.b +ETT_{min}(l, s) \leq T_{lv}(l, s, tr). \\
  &(i) x.e-ETE_{min}(l, s) \leq T_{arrv}(l, s, tr). \\
 &(iii)T_{lv}(l', s, tr')-T_{arrv}(l, s, tr) \geq TFT_{min}(l, l', s). \\
\end{split}
\label{equ:condition}
\end{equation}

For a passenger, given a route, we can find all plans chosen during her/his trip by Equation~(\ref{equ:condition}). As in Figure~\ref{fig:mutilroute}(b), for a passenger who taps-in at station $O$ at time point $T1$ and taps-out at station $D$ at time point $T2$, if he chooses the first route, he may choose plan $\{tr_i,tr_j\}$ or $\{tr_{i+1},tr_j\}$. If he chooses the second route, he may choose plan $\{tr_i,tr_k\}$. It is to be noted that, upon our two assumptions above, the train chosen by passenger before he/she exiting metro system can be uniquely inferred.

